Deep Data Flow Analysis

Compiler architects increasingly look to machine learning when building heuristics for compiler optimization. The promise of automatic heuristic design, freeing the compiler engineer from the complex interactions of program, architecture, and other optimizations, is alluring. However, most machine learning methods cannot replicate even the simplest of the abstract interpretations of data flow analysis that are critical to making good optimization decisions. This must change for machine learning to become the dominant technology in compiler heuristics. To this end, we propose ProGraML - Program Graphs for Machine Learning - a language-independent, portable representation of whole-program semantics for deep learning. To benchmark current and future learning techniques for compiler analyses we introduce an open dataset of 461k Intermediate Representation (IR) files for LLVM, covering five source programming languages, and 15.4M corresponding data flow results. We formulate data flow analysis as an MPNN and show that, using ProGraML, standard analyses can be learned, yielding improved performance on downstream compiler optimization tasks.

==> main.tex <==
\title{Deep Data Flow Analysis}

\maketitle
\begin{abstract}
\input{abstract}
\end{abstract}


\input{sections/introduction}
\input{sections/related_work}
\input{sections/representation}
\input{sections/machine_learning}
\input{sections/data_flow_experiments}
\input{sections/conclusion}
% \clearpage
% \input{sections/broader_impact}

\bibliography{refs}
\bibliographystyle{iclr2021_conference}


==> sections/broader_impact.tex <==
\section*{Broader Impact}

This paper directly concerns the automation of compiler construction using deep learning. 
In the compiler community, there is a widely held view that the topic is ethically neutral. In fact, there is little if any literature on the topic. This view is mirrored by research funding agencies ethical review processes. A brief review of publicly visible research projects funded by the US and EU shows that compiler projects are deemed as having no ethical issues.
This paper improves a tool that can be used for all applications both good and bad. 

However, if we were to completely automate compiler construction, then potentially existing highly skilled compiler engineers will be made redundant or their jobs deskilled. In reality, compiler engineers are often tied up with the complex interaction between different compiler passes and software engineering issues, preventing them from aggressively exploiting hardware potential. As hardware becomes increasingly heterogeneous, this is a growing problem. Greater automation allows them to focus on deeper more challenging issues.

Given that compiler construction is one of the more complex programming tasks, its complete automation   implies that  program generation for more straightforward tasks is also 
possible. While the number of compiler engineers is relatively small, application programmers are a much wider class of individuals who may be adversely affected by automation.

This perceived threat  of program automation has a long history. The first FORTRAN compiler was thought to eliminate real coding with a user friendly high level language. In the 1980s, fifth generation languages were considered a threat to the large numbers of procedural programmers.
In fact,  advances in program  automation have  allowed  programmers
to focus on ever more complex applications rather than  details of the underlying system. 
The ability to further automate compiler construction lowers the bar to the exploration of new programming languages 
and hence new application areas. It enhances programmer productivity  and creativity.


==> supplementary_material.tex <==
\title{Deep Data Flow: Appendices}

\maketitle

\appendix
\input{appendix/dataflow_problems}
\input{appendix/dataset}
\input{appendix/experimental_setup}
\input{appendix/downstream_tasks}

\bibliography{refs}
\bibliographystyle{iclr2021_conference}


==> tables/confusion_matrices.tex <==
\centering
\scriptsize
\renewcommand{\arraystretch}{1.5}
\begin{subfigure}{.22\linewidth}
	\centering
	\begin{tabular}{r | c c}
		\toprule
		& $\bm{P_-}$ & $\bm{P_+}$ \\
		\midrule
		$\bm{T_-}$ & 96.64\% & 0.01\% \\
		$\bm{T_+}$ & 0.01\% & 3.34\% \\
		\bottomrule
	\end{tabular}
	\caption{\textsc{Reachability}}
\end{subfigure}
% \hfill
\begin{subfigure}{.17\linewidth}
	\centering
	\begin{tabular}{| c c}
		\toprule
		$\bm{P_-}$ & $\bm{P_+}$ \\
		\midrule
		95.94\% & 0.13\% \\
		1.70\% & 2.23\% \\
		\bottomrule
	\end{tabular}
	\caption{\textsc{Dominance}}
\end{subfigure}
% \hfill
\begin{subfigure}{.17\linewidth}
	\begin{tabular}{| c c}
		\toprule
		$\bm{P_-}$ & $\bm{P_+}$ \\
		\midrule
		98.80\% & 0.00\% \\
		0.00\% & 1.20 \% \\
		\bottomrule
	\end{tabular}
	\caption{\textsc{DataDep}}
\end{subfigure}
% \hfill
\begin{subfigure}{.17\linewidth}
	\centering
	\begin{tabular}{| c c}
		\toprule
		$\bm{P_-}$ & $\bm{P_+}$ \\
		\midrule
		90.00\% & 0.00\% \\
		0.00\% & 9.99\% \\
		\bottomrule
	\end{tabular}
	\caption{\textsc{Liveness}}
\end{subfigure}
% \hfill
\begin{subfigure}{.21\linewidth}
	\begin{tabular}{| c c}
		\toprule
		$\bm{P_-}$ & $\bm{P_+}$ \\
		\midrule
		99.12\% & 0.02\% \\
		0.13\% & 0.73\% \\
		\bottomrule
	\end{tabular}
	\caption{\textsc{Subexpressions}}
\end{subfigure}
